Cubing for Tuning

We are exploring the problem of building an automated reasoning procedure that adaptively tunes the high-level solving strategy for a given problem. There are two main distinctive characteristics of our approach: tuning is performed solely online, unlike the common use of tuning as an offline process; and tuning data comes exclusively from the given instance, so we do not rely on the availability of similar benchmarks and can work with unique challenging instances. Our approach builds on top of the divide-and-conquer paradigm that naturally serves partitioned sub-problems for an automated tuning algorithm to obtain a good solving strategy. We demonstrate performance improvement on two classes of important problems--SAT-solving and neural network verification--and show that our method can learn unconventional solving strategies in some cases.

==> tabs/detailed_results_sc24.tex <==
\begin{center}
\scriptsize
\setlength{\tabcolsep}{10.3pt}
\begin{xltabular}{\textwidth}{@{}lrrrrrr@{}}
\toprule
& \multicolumn{2}{c}{\tabtitle{\cnc}} & \multicolumn{2}{c}{\tabtitle{\cncTuneAndVal}} & \multicolumn{2}{c}{\tabtitle{\painless}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\tabtitle{Benchmark}  & \tabtitle{Res.} & \coltimetotal & \tabtitle{Res.} & \coltimetotal & \tabtitle{Res.} & \coltimetotal  \\
\endhead
002 & SAT & 160.54 & SAT & 280.54 & SAT & 640.05 \\
004 & SAT & 13.18 & SAT & 133.18 & SAT & 10.04 \\
128\_100 & MO & 838.48 & MO & 816.91 & SAT & 167.81 \\
128\_125 & MO & 1084.30 & MO & 1050.09 & UNK & 115.54 \\
128\_75 & MO & 614.81 & MO & 610.58 & SAT & 557.48 \\
170058440 & SAT & 1978.07 & SAT & 12.63 & SAT & 0.97 \\
1\_ET\_256\_K\_55 & TO & 3601.30 & TO & 3601.29 & TO & 3601.31 \\
1\_ET\_256\_K\_70 & UNS & 984.24 & UNS & 548.70 & UNS & 13.14 \\
1\_ET\_512\_K\_110 & TO & 3601.31 & TO & 3601.32 & TO & 3601.31 \\
1\_ET\_512\_K\_96 & TO & 3601.32 & TO & 3721.32 & SAT & 427.77 \\
1\_TC\_256\_K\_64 & UNS & 1998.09 & UNS & 1245.00 & UNS & 281.77 \\
1\_TC\_256\_K\_68 & UNS & 1272.73 & UNS & 700.64 & UNS & 30.50 \\
1\_TC\_256\_K\_71 & UNS & 1130.14 & UNS & 628.34 & UNS & 13.10 \\
1\_ZC\_1024\_K\_116 & TO & 3601.31 & TO & 3601.30 & TO & 3601.29 \\
1\_ZC\_1024\_K\_117 & TO & 3601.34 & TO & 3601.33 & TO & 3601.30 \\
1\_ZC\_512\_K\_60 & SAT & 122.24 & SAT & 242.24 & SAT & 66.30 \\
1\_ZC\_512\_K\_61 & SAT & 139.94 & SAT & 259.94 & SAT & 28.80 \\
1\_ZC\_512\_K\_63 & TO & 3601.31 & TO & 3721.31 & TO & 3601.30 \\
1\_ZC\_512\_K\_64 & TO & 3601.31 & TO & 3721.31 & TO & 3601.31 \\
1\_ZC\_512\_K\_65 & TO & 3601.31 & TO & 3721.31 & TO & 3601.29 \\
1\_ZC\_512\_K\_67 & TO & 3601.31 & TO & 3721.31 & TO & 3601.31 \\
2dlx\_ca\_bp\_f\_liveness & TO & 3601.33 & TO & 3601.29 & TO & 3601.29 \\
32\_100 & MO & 252.34 & MO & 245.49 & SAT & 70.97 \\
32\_200 & MO & 468.23 & MO & 461.20 & SAT & 42.70 \\
32\_325 & MO & 762.59 & MO & 754.19 & UNK & 468.58 \\
32\_350 & MO & 844.92 & MO & 808.72 & UNK & 218.47 \\
64\_150 & MO & 645.63 & MO & 610.99 & SAT & 47.01 \\
64\_200 & MO & 798.04 & MO & 821.81 & SAT & 69.84 \\
64\_25 & SAT & 167.89 & SAT & 169.54 & SAT & 7.36 \\
6g\_6color\_366\_050\_04 & SAT & 636.57 & SAT & 756.57 & SAT & 12.04 \\
6s130\_opt & UNS & 1733.94 & UNS & 1624.34 & UNS & 71.39 \\
6s167\_opt & UNS & 11.15 & UNS & 18.16 & UNS & 0.68 \\
af\_synthesis\_stb\_50\_100\_4\_sat & UNS & 25.36 & UNS & 25.27 & SAT & 55.45 \\
af\_synthesis\_stb\_50\_100\_9\_sat & ERR & 9.47 & ERR & 9.59 & SAT & 4.60 \\
af\_synthesis\_stb\_50\_100\_9\_unsat & ERR & 9.44 & ERR & 9.68 & UNS & 144.24 \\
af\_synthesis\_stb\_50\_120\_4\_sat & ERR & 10.51 & ERR & 10.84 & SAT & 28.75 \\
af\_synthesis\_stb\_50\_140\_0\_unsat & UNS & 20.24 & UNS & 22.09 & UNS & 154.15 \\
af\_synthesis\_stb\_50\_140\_1\_unsat & ERR & 10.21 & ERR & 10.49 & UNS & 259.23 \\
af\_synthesis\_stb\_50\_140\_3\_unsat & ERR & 10.47 & ERR & 10.06 & UNS & 54.03 \\
af\_synthesis\_stb\_50\_200\_0\_sat & SAT & 159.50 & SAT & 207.34 & SAT & 22.89 \\
af\_synthesis\_stb\_50\_200\_0\_unsat & UNS & 686.37 & UNS & 739.37 & UNS & 139.76 \\
af\_synthesis\_stb\_50\_200\_4\_unsat & UNS & 26.25 & UNS & 29.30 & UNS & 69.61 \\
af\_synthesis\_stb\_50\_40\_2\_unsat & ERR & 3.68 & ERR & 3.98 & UNS & 92.28 \\
af\_synthesis\_stb\_50\_40\_9\_sat & TO & 3601.30 & TO & 3601.29 & SAT & 97.10 \\
af\_synthesis\_stb\_50\_40\_9\_unsat & TO & 3601.29 & TO & 3601.29 & UNS & 321.46 \\
apn\_sbox5\_cut3\_symmbreak & TO & 3601.29 & SAT & 2716.09 & TO & 3601.32 \\
asconhashv12\_opt64\_H11\_M2\_fCHjS2L0du5\_m2\_4.c & UNS & 415.27 & UNS & 438.64 & SAT & 14.84 \\
asconhashv12\_opt64\_H11\_M2\_MxJOnbQIXNd\_m5\_6.c & SAT & 208.24 & SAT & 328.24 & SAT & 13.05 \\
asconhashv12\_opt64\_H11\_M2\_tBi5i1RIgRz\_m0\_1\_U23.c & UNS & 511.47 & UNS & 506.06 & UNS & 131.24 \\
asconhashv12\_opt64\_H5\_M2\_xEJ8F\_m0\_3\_U5.c & UNS & 265.39 & UNS & 385.39 & UNS & 44.65 \\
asconhashv12\_opt64\_H6\_M2\_PgbpwX\_m0\_4\_U1.c & UNS & 278.30 & UNS & 398.30 & UNS & 52.97 \\
asconhashv12\_opt64\_H9\_M2\_MIC4kfhiA\_m0\_6\_U2.c & UNS & 514.18 & UNS & 515.04 & UNS & 128.14 \\
atco\_enc1\_opt1\_10\_15 & SAT & 150.28 & SAT & 270.28 & SAT & 7.91 \\
barman\_pfile06\_022.sas.ex.7 & UNS & 100.04 & UNS & 105.85 & UNS & 1.11 \\
battleship\_14\_26\_sat & SAT & 1.16 & SAT & 0.94 & SAT & 0.80 \\
bmc\_QICE\_snp\_vld\_30 & TO & 3601.33 & TO & 3601.37 & UNS & 85.36 \\
bphp\_p23\_h22 & TO & 3601.33 & TO & 3601.32 & TO & 3601.31 \\
Break\_08\_24.xml & SAT & 0.80 & SAT & 0.94 & SAT & 0.19 \\
Break\_18\_32.xml & SAT & 1720.96 & SAT & 1840.96 & SAT & 1680.94 \\
Break\_20\_72.xml & SAT & 2043.03 & SAT & 2163.03 & SAT & 531.83 \\
Break\_triple\_20\_36.xml & TO & 3601.31 & TO & 3601.32 & TO & 3601.31 \\
Break\_unsat\_04\_03.xml & UNS & 0.31 & UNS & 0.39 & UNS & 0.04 \\
Break\_unsat\_06\_07.xml & UNS & 6.54 & UNS & 15.27 & UNS & 0.68 \\
Break\_unsat\_14\_23.xml & TO & 3601.30 & TO & 3601.32 & TO & 3601.29 \\
Break\_unsat\_16\_27.xml & TO & 3601.31 & TO & 3601.32 & TO & 3601.29 \\
Break\_unsat\_18\_31.xml & TO & 3601.32 & TO & 3721.32 & TO & 3601.30 \\
bvsub\_19952.smt2 & TO & 3601.30 & TO & 3601.33 & UNS & 951.86 \\
circuit\_32in32out\_100gates\_7in7out\_64\_seed2 & SAT & 1113.95 & SAT & 1134.45 & SAT & 63.99 \\
circuit\_32in32out\_350gates\_6in6out\_64\_seed1 & TO & 3601.31 & TO & 3601.31 & SAT & 47.09 \\
circuit\_32in32out\_400gates\_6in6out\_64\_seed1 & SAT & 225.84 & SAT & 345.84 & SAT & 173.31 \\
circuit\_32in32out\_500gates\_6in6out\_64\_seed1 & TO & 3601.31 & TO & 3601.31 & SAT & 504.53 \\
circuit\_32in32out\_64gates\_8in6out\_128\_seed2 & TO & 3601.31 & TO & 3601.34 & SAT & 762.13 \\
circuit\_32in32out\_70gates\_7in7out\_128\_seed1 & TO & 3601.30 & TO & 3601.31 & SAT & 898.47 \\
circuit\_32in32out\_80gates\_7in7out\_128\_seed1 & SAT & 2064.94 & SAT & 2184.94 & SAT & 407.23 \\
circuit\_32in32out\_96gates\_7in7out\_128\_seed1 & TO & 3601.30 & TO & 3601.30 & SAT & 1588.96 \\
circuit\_32in64out\_150gates\_6in6out\_256\_seed1 & TO & 3601.31 & TO & 3601.30 & TO & 3601.32 \\
circuit\_48in24out\_100gates\_7in7out\_128\_seed1 & SAT & 819.76 & SAT & 939.76 & SAT & 374.16 \\
circuit\_48in64out\_1000gates\_4in4out\_128\_seed4 & SAT & 47.98 & SAT & 96.08 & SAT & 23.50 \\
circuit\_48in64out\_700gates\_4in4out\_128\_seed1 & SAT & 31.97 & SAT & 60.05 & SAT & 5.07 \\
circuit\_48in64out\_800gates\_4in4out\_128\_seed1 & SAT & 20.86 & SAT & 140.86 & SAT & 10.63 \\
circuit\_48in64out\_800gates\_4in4out\_128\_seed4 & SAT & 7.00 & SAT & 127.00 & SAT & 6.90 \\
circuit\_64in64out\_64gates\_8in5out\_256\_seed1 & SAT & 383.88 & SAT & 453.95 & SAT & 10.87 \\
Circuit\_multiplier22 & SAT & 17.61 & SAT & 115.89 & SAT & 52.70 \\
cliquecolouring\_n13\_k8\_c7 & TO & 3601.30 & TO & 3601.32 & TO & 3601.29 \\
cliquecolouring\_n13\_k9\_c8 & TO & 3601.30 & TO & 3601.31 & TO & 3601.31 \\
cliquecolouring\_n15\_k9\_c8 & TO & 3601.31 & TO & 3601.32 & TO & 3601.29 \\
cliquecolouring\_n21\_k6\_c5 & TO & 3601.29 & TO & 3601.33 & TO & 3601.32 \\
cliquecolouring\_n31\_k5\_c4 & TO & 3601.31 & TO & 3601.31 & TO & 3601.31 \\
cliquecolouring\_n41\_k5\_c4 & TO & 3601.31 & TO & 3601.32 & TO & 3601.30 \\
clique\_n2\_k10 & UNS & 12.39 & UNS & 27.61 & UNS & 4.38 \\
combined\_crypto1\_wff\_seed\_102\_wffvars\_500 & SAT & 14.86 & SAT & 134.86 & SAT & 1.53 \\
combined\_crypto1\_wff\_seed\_1\_wffvars\_450 & SAT & 3.26 & SAT & 93.25 & SAT & 1.67 \\
constraints\_16\_0.3\_1 & UNS & 33.25 & UNS & 70.24 & UNS & 40.46 \\
constraints\_16\_0.4\_1 & UNS & 49.76 & UNS & 102.44 & UNS & 26.74 \\
constraints\_16\_0.5\_1 & UNS & 59.26 & UNS & 122.44 & UNS & 25.90 \\
constraints\_17\_0.3\_2 & UNS & 57.14 & UNS & 104.87 & UNS & 15.28 \\
constraints\_17\_0.4\_1 & SAT & 135.05 & SAT & 136.89 & SAT & 2.98 \\
constraints\_17\_0.4\_2 & UNS & 77.76 & UNS & 151.97 & UNS & 17.93 \\
constraints\_17\_0.5\_2 & UNS & 108.64 & UNS & 166.94 & UNS & 26.27 \\
constraints\_18\_0.3\_2 & UNS & 149.93 & UNS & 222.75 & UNS & 76.43 \\
constraints\_18\_0.4\_2 & UNS & 371.94 & UNS & 491.94 & UNS & 132.34 \\
constraints\_18\_0.5\_2 & UNS & 461.25 & UNS & 581.25 & UNS & 163.59 \\
constraints\_25\_4\_5\_12\_12\_0\_0\_0 & UNS & 126.94 & UNS & 162.46 & UNS & 46.18 \\
crafted\_n12\_d6\_c4\_num23 & UNS & 458.36 & UNS & 471.96 & UNS & 73.46 \\
crn\_11\_99\_u & UNS & 230.50 & UNS & 261.14 & UNS & 0.44 \\
ctl\_4201\_555\_unsat\_pre & TO & 3601.34 & TO & 3721.34 & UNS & 255.79 \\
ctl\_4291\_567\_2\_unsat\_sc2013 & TO & 3601.31 & TO & 3721.31 & UNS & 379.33 \\
ctl\_4291\_567\_9\_unsat & UNS & 3249.15 & UNS & 3369.15 & UNS & 118.90 \\
DLTM\_twitter774\_83\_17 & SAT & 445.54 & SAT & 565.54 & SAT & 21.38 \\
Dodecahedron\_k7 & TO & 3601.30 & TO & 3721.30 & UNS & 2487.80 \\
ecarev\_110\_4099\_22\_30\_7 & SAT & 260.65 & SAT & 287.40 & SAT & 151.08 \\
EDP3\_11000 & SAT & 25.70 & SAT & 145.70 & SAT & 23.70 \\
ER\_400\_20\_4.apx\_1\_DC\_AD & UNS & 39.06 & UNS & 59.94 & UNS & 90.36 \\
ER\_400\_20\_4.apx\_2\_DC\_AD & UNS & 106.17 & UNS & 68.54 & UNS & 81.10 \\
ER\_400\_20\_4.apx\_2\_DC\_ST & UNS & 36.34 & UNS & 36.29 & UNS & 70.11 \\
ER\_400\_20\_7.apx\_1\_DC\_AD & UNS & 184.01 & UNS & 66.17 & UNS & 167.01 \\
ER\_400\_20\_7.apx\_2\_DC\_AD & UNS & 724.96 & UNS & 385.24 & UNS & 743.18 \\
ER\_400\_20\_7.apx\_2\_DC\_ST & UNS & 347.99 & UNS & 204.60 & UNS & 571.04 \\
ER\_500\_30\_3.apx\_1\_DC\_ST & UNS & 93.84 & UNS & 57.60 & UNS & 74.08 \\
ER\_500\_30\_3.apx\_2\_DC\_AD & UNS & 396.41 & UNS & 242.61 & UNS & 208.61 \\
ex065\_25 & SAT & 25.56 & SAT & 96.89 & SAT & 2.63 \\
exam\_flat\_0.04\_2018\_3 & SAT & 433.50 & SAT & 509.34 & SAT & 141.46 \\
f9idw & UNS & 1997.66 & UNS & 2053.36 & UNS & 53.73 \\
fermat\_931960058139995587 & TO & 3601.30 & SAT & 2446.15 & TO & 3601.27 \\
fixedbandwidth\_eq\_31\_shuffled & UNS & 603.21 & UNS & 821.88 & UNS & 257.03 \\
FmlaEquivChain\_4\_6\_6 & TO & 3601.32 & TO & 3601.31 & UNS & 9.43 \\
FmlaEquivChain\_4\_8\_8 & TO & 3601.32 & TO & 3601.31 & UNS & 698.91 \\
FmlaImplyChain\_3\_7\_7 & UNS & 2436.23 & UNS & 2542.61 & UNS & 53.27 \\
FmlaImplyChain\_3\_7\_8 & TO & 3601.31 & TO & 3601.31 & UNS & 1453.84 \\
Folkman\_175\_1251868 & SAT & 37.47 & SAT & 125.00 & SAT & 0.47 \\
Folkman\_175\_7416734 & SAT & 36.37 & SAT & 122.40 & SAT & 0.65 \\
Folkman\_175\_9054056 & SAT & 69.94 & SAT & 156.65 & SAT & 0.77 \\
Folkman\_180\_11710376 & SAT & 69.23 & SAT & 155.54 & SAT & 0.49 \\
Folkman\_180\_5383714 & SAT & 38.87 & SAT & 129.36 & SAT & 0.90 \\
Folkman\_185\_152478531 & SAT & 118.64 & SAT & 202.04 & SAT & 7.49 \\
Folkman\_185\_19924337 & SAT & 66.55 & SAT & 158.16 & SAT & 0.53 \\
Folkman\_185\_75415683 & SAT & 64.38 & SAT & 153.13 & SAT & 0.28 \\
Folkman\_190\_104806020 & SAT & 189.07 & SAT & 271.19 & SAT & 22.53 \\
Folkman\_190\_358004741 & SAT & 386.96 & SAT & 485.94 & SAT & 4.58 \\
Folkman\_190\_66337703 & SAT & 331.68 & SAT & 406.55 & SAT & 2.83 \\
frb45\_21\_2.used\_as.sat04\_884 & SAT & 395.14 & SAT & 186.38 & SAT & 61.71 \\
frb65\_12\_2.used\_as.sat04\_874 & SAT & 8.17 & SAT & 34.64 & SAT & 1.83 \\
g2\_ak128boothbg2msaig & TO & 3601.30 & TO & 3721.30 & TO & 3601.29 \\
g2\_ak128boothbg2msisc & TO & 3601.30 & TO & 3721.30 & SAT & 1415.34 \\
g2\_hwmcc15deep\_6s161\_k17 & UNS & 548.14 & UNS & 786.64 & UNS & 349.43 \\
g2\_hwmcc15deep\_bob12s02\_k16 & TO & 3601.33 & TO & 3601.32 & UNS & 2453.13 \\
g2\_slp\_synthesis\_aes\_top30 & SAT & 129.08 & SAT & 249.08 & SAT & 16.66 \\
g2\_T93.2.1 & TO & 3601.32 & TO & 3601.32 & UNS & 244.53 \\
g2\_test\_v5\_r10\_vr10\_c1\_s21502.smt2\_cvc4 & UNS & 2254.27 & UNS & 2248.44 & UNS & 142.74 \\
goldcrest\_and\_9 & UNS & 2376.35 & UNS & 2472.04 & UNS & 59.05 \\
GracefulGraph\_K05\_P02\_c18 & SAT & 7.18 & SAT & 53.70 & SAT & 2.19 \\
grs\_64\_128 & UNS & 186.33 & UNS & 250.34 & UNS & 951.79 \\
grs\_64\_64 & UNS & 66.19 & UNS & 143.94 & UNS & 91.08 \\
HCP\_446\_105 & SAT & 580.94 & SAT & 604.70 & SAT & 409.51 \\
hcp\_CP18\_18 & TO & 3601.31 & TO & 3601.32 & SAT & 401.49 \\
hwb\_n24\_02\_S786928571.shuffled\_as.sat03\_1618 & UNS & 21.68 & UNS & 24.48 & UNS & 71.63 \\
hwmcc12miters\_xits\_iso\_6s111 & TO & 3601.30 & TO & 3601.32 & TO & 3601.29 \\
hwmcc17miters\_xits\_iso\_6s281b35 & TO & 3601.32 & TO & 3601.30 & TO & 3601.30 \\
hwmcc17miters\_xits\_iso\_bobsmfpu & TO & 3601.31 & TO & 3601.30 & TO & 3601.29 \\
hwmcc17miters\_xits\_iso\_oski15a08b00s & TO & 3601.30 & TO & 3601.34 & UNS & 3588.27 \\
hwmcc17miters\_xits\_iso\_oski15a08b08s & TO & 3601.31 & TO & 3601.34 & UNS & 3455.73 \\
hwmcc20miters\_iso\_mul2 & TO & 3601.31 & TO & 3601.31 & TO & 3601.30 \\
hwmcc20miters\_iso\_mul3 & TO & 3601.32 & TO & 3601.32 & TO & 3601.29 \\
hwmcc20miters\_iso\_mul7 & TO & 3601.30 & TO & 3601.31 & TO & 3601.30 \\
hwmcc20miters\_iso\_rast\_p06 & TO & 3601.30 & TO & 3721.30 & TO & 3601.31 \\
hwmcc20miters\_iso\_rast\_p11 & TO & 3601.30 & TO & 3721.30 & TO & 3601.32 \\
IBM\_FV\_2004\_rule\_batch\_1\_31\_1\_SAT\_dat.k40 & UNS & 417.36 & UNS & 461.87 & UNS & 224.83 \\
ITC2021\_Early\_10.xml & TO & 3601.33 & TO & 3601.30 & SAT & 1343.93 \\
ITC2021\_Early\_3.xml & SAT & 6.88 & SAT & 7.05 & SAT & 0.27 \\
ITC2021\_Middle\_1.xml & TO & 3601.31 & TO & 3601.30 & TO & 3601.30 \\
j3037\_10\_mdd\_b & SAT & 5.94 & SAT & 108.45 & SAT & 2.97 \\
j3037\_10\_mdd\_bm1 & UNS & 46.44 & UNS & 104.70 & UNS & 13.27 \\
j3037\_10\_rggt\_b & SAT & 7.86 & SAT & 70.09 & SAT & 2.53 \\
j3037\_1\_gmto\_b & SAT & 43.76 & SAT & 80.54 & SAT & 11.58 \\
j3037\_1\_mdd\_b & SAT & 17.18 & SAT & 128.64 & SAT & 20.81 \\
j3037\_9\_mdd\_bm1 & UNS & 1390.94 & UNS & 1424.73 & TO & 3601.32 \\
j3037\_9\_rggt\_b & SAT & 79.27 & SAT & 196.76 & SAT & 6.90 \\
j3045\_10\_gmto\_b & SAT & 111.57 & SAT & 211.70 & SAT & 30.50 \\
j3045\_10\_rggt\_b & SAT & 60.19 & SAT & 140.21 & SAT & 23.66 \\
j3045\_4\_gmto\_b & SAT & 252.74 & SAT & 275.09 & SAT & 36.69 \\
j3045\_4\_mdd\_bm1 & UNS & 121.24 & UNS & 165.04 & UNS & 159.80 \\
jgiraldezlevy.2200.9086.08.40.41 & SAT & 159.44 & SAT & 228.54 & SAT & 6.53 \\
Kakuro\_easy\_097\_ext.xml.hg\_4 & TO & 3601.32 & TO & 3601.33 & UNS & 328.05 \\
lec\_mult\_CvD\_11x11 & UNS & 42.56 & UNS & 47.54 & UNS & 279.96 \\
lec\_mult\_CvK\_11x10 & UNS & 34.84 & UNS & 50.74 & UNS & 143.61 \\
lec\_mult\_CvK\_11x11 & UNS & 63.74 & UNS & 94.76 & UNS & 359.28 \\
lec\_mult\_CvK\_12x11 & UNS & 105.39 & UNS & 132.05 & UNS & 967.13 \\
lec\_mult\_CvK\_12x12 & UNS & 217.65 & UNS & 251.26 & UNS & 2619.90 \\
lec\_mult\_CvW\_12x11 & UNS & 68.90 & UNS & 84.55 & UNS & 663.58 \\
lec\_mult\_CvW\_12x12 & UNS & 139.04 & UNS & 175.47 & UNS & 2050.09 \\
lec\_mult\_DvK\_11x10 & UNS & 35.54 & UNS & 48.10 & UNS & 136.66 \\
lec\_mult\_DvK\_12x12 & UNS & 232.76 & UNS & 260.54 & UNS & 2896.36 \\
lec\_mult\_DvW\_11x10 & UNS & 22.00 & UNS & 32.51 & UNS & 120.51 \\
lec\_mult\_DvW\_12x11 & UNS & 68.57 & UNS & 86.94 & UNS & 913.34 \\
lec\_mult\_DvW\_12x12 & UNS & 139.56 & UNS & 173.97 & UNS & 2428.66 \\
lec\_mult\_KvW\_10x10 & UNS & 23.90 & UNS & 38.70 & UNS & 58.84 \\
lec\_mult\_KvW\_11x10 & UNS & 36.04 & UNS & 54.53 & UNS & 140.93 \\
lec\_mult\_KvW\_12x11 & UNS & 113.24 & UNS & 141.18 & UNS & 1065.63 \\
linked\_list\_swap\_contents\_safety\_unwind45 & ERR & 294.74 & ERR & 290.60 & UNS & 16.74 \\
linked\_list\_swap\_contents\_safety\_unwind54 & ERR & 578.24 & ERR & 574.27 & UNS & 37.78 \\
linked\_list\_swap\_contents\_safety\_unwind57 & TO & 3601.32 & TO & 3601.33 & UNS & 47.58 \\
linked\_list\_swap\_contents\_safety\_unwind62 & MO & 338.53 & MO & 338.44 & UNS & 54.55 \\
linked\_list\_swap\_contents\_safety\_unwind63 & MO & 321.57 & MO & 320.68 & UNS & 38.78 \\
linked\_list\_swap\_contents\_safety\_unwind65 & ERR & 671.05 & ERR & 670.76 & UNS & 93.33 \\
linked\_list\_swap\_contents\_safety\_unwind68 & MO & 315.74 & MO & 310.24 & UNS & 39.38 \\
linked\_list\_swap\_contents\_safety\_unwind69 & MO & 345.92 & MO & 342.25 & UNS & 106.43 \\
linked\_list\_swap\_contents\_safety\_unwind70 & MO & 332.83 & MO & 332.93 & UNS & 60.60 \\
linked\_list\_swap\_contents\_safety\_unwind73 & MO & 362.76 & MO & 365.24 & UNS & 103.43 \\
linked\_list\_swap\_contents\_safety\_unwind76 & MO & 392.59 & MO & 386.97 & UNS & 38.69 \\
linked\_list\_swap\_contents\_safety\_unwind78 & MO & 414.88 & MO & 408.96 & UNS & 110.79 \\
linked\_list\_swap\_contents\_safety\_unwind80 & MO & 453.24 & MO & 452.83 & UNS & 167.08 \\
lru\_10 & ERR & 462.24 & ERR & 452.94 & SAT & 67.15 \\
lru\_6 & ERR & 273.61 & ERR & 274.15 & SAT & 43.23 \\
lru\_7 & ERR & 319.78 & ERR & 314.28 & SAT & 48.91 \\
lru\_8 & ERR & 364.06 & ERR & 356.09 & SAT & 55.03 \\
lru\_9 & ERR & 419.30 & ERR & 419.69 & SAT & 65.53 \\
manol\_pipe\_g10bid\_i & UNS & 1315.59 & UNS & 1359.54 & UNS & 35.80 \\
marg5x5.shuffled\_as.sat03\_1455 & TO & 3601.30 & TO & 3601.31 & UNS & 0.02 \\
MASG0\_72\_keystream76\_0 & SAT & 202.81 & SAT & 322.81 & SAT & 59.49 \\
mchess\_15 & UNS & 3296.14 & UNS & 3313.84 & UNS & 25.13 \\
mchess\_16 & TO & 3601.30 & TO & 3601.30 & UNS & 25.97 \\
mchess\_17 & TO & 3601.29 & TO & 3601.32 & UNS & 476.98 \\
md5\_48\_1 & SAT & 103.88 & SAT & 223.88 & SAT & 49.03 \\
mdp\_28\_10\_unsat & UNS & 147.25 & UNS & 156.16 & UNS & 355.34 \\
mdp\_28\_11\_sat & SAT & 81.44 & SAT & 90.19 & SAT & 3.26 \\
mdp\_28\_14\_sat & SAT & 12.74 & SAT & 31.77 & SAT & 7.76 \\
mdp\_28\_14\_unsat & UNS & 196.54 & UNS & 199.21 & UNS & 640.53 \\
mdp\_28\_16\_unsat & UNS & 184.58 & UNS & 187.64 & UNS & 603.13 \\
mdp\_32\_10\_sat & SAT & 1178.31 & SAT & 1211.74 & SAT & 385.44 \\
mdp\_32\_10\_unsat & TO & 3601.30 & TO & 3601.29 & TO & 3601.31 \\
mdp\_32\_11\_sat & TO & 3601.29 & TO & 3601.30 & SAT & 549.69 \\
mdp\_32\_11\_unsat & TO & 3601.30 & TO & 3601.31 & TO & 3601.30 \\
mdp\_32\_12\_unsat & TO & 3601.31 & TO & 3601.29 & TO & 3601.31 \\
mdp\_32\_14\_sat & SAT & 2129.68 & SAT & 2526.44 & TO & 3601.30 \\
mdp\_32\_14\_unsat & TO & 3601.29 & UNS & 3426.14 & TO & 3601.31 \\
mdp\_32\_16\_sat & SAT & 306.19 & SAT & 442.27 & SAT & 178.63 \\
mdp\_36\_10\_sat & TO & 3601.29 & TO & 3601.32 & TO & 3601.30 \\
mdp\_36\_10\_unsat & TO & 3601.31 & TO & 3601.32 & TO & 3601.30 \\
mdp\_36\_12\_unsat & TO & 3601.29 & TO & 3601.30 & TO & 3601.31 \\
mdp\_36\_14\_sat & TO & 3601.32 & TO & 3601.31 & TO & 3601.28 \\
mp1\_blockpuzzle\_5x10\_s7\_free4 & UNS & 87.24 & UNS & 131.04 & UNS & 114.46 \\
mp1\_klieber2017s\_0500\_023\_t12 & SAT & 44.99 & SAT & 44.24 & SAT & 5.47 \\
mp1\_Nb5T15 & SAT & 53.95 & SAT & 9.80 & SAT & 8.03 \\
mp1\_Nb7T42 & SAT & 14.07 & SAT & 83.79 & SAT & 2.07 \\
mp1\_ps\_5000\_21250\_3\_0\_0.8\_0\_1.50\_6 & UNS & 19.54 & UNS & 41.84 & UNS & 15.43 \\
mrpp\_4x4\#12\_12 & UNS & 197.00 & UNS & 141.45 & UNS & 2.27 \\
mulhs016\_sc2009 & TO & 3601.31 & TO & 3601.30 & TO & 3601.32 \\
Nb13T165 & TO & 3601.31 & SAT & 139.03 & SAT & 536.90 \\
Nb44T6 & TO & 3601.33 & TO & 3601.34 & UNS & 695.47 \\
noL\_11\_0 & SAT & 362.18 & SAT & 406.09 & SAT & 23.89 \\
noL\_11\_10 & TO & 3601.31 & TO & 3601.30 & SAT & 3.34 \\
noL\_11\_12 & TO & 3601.30 & TO & 3601.30 & SAT & 0.64 \\
noL\_11\_14 & TO & 3601.30 & TO & 3601.31 & SAT & 2.36 \\
noL\_11\_16 & TO & 3601.33 & TO & 3601.29 & SAT & 0.27 \\
noL\_11\_18 & TO & 3601.31 & TO & 3601.31 & SAT & 8.00 \\
noL\_11\_20 & TO & 3601.32 & TO & 3601.31 & SAT & 0.15 \\
noL\_11\_2 & TO & 3601.30 & TO & 3601.31 & SAT & 11.80 \\
noL\_11\_4 & TO & 3601.30 & TO & 3601.31 & SAT & 12.66 \\
noL\_11\_6 & TO & 3601.31 & TO & 3601.30 & SAT & 7.94 \\
noL\_11\_8 & TO & 3601.32 & TO & 3601.30 & SAT & 4.69 \\
oisc\_subrv\_sll\_nested\_11 & MO & 638.90 & MO & 643.79 & UNS & 1049.63 \\
oisc\_subrv\_sll\_nested\_13 & MO & 846.55 & MO & 885.87 & UNS & 1698.59 \\
openstacks\_sequencedstrips\_nonadl\_nonnegated... & UNS & 1007.54 & UNS & 855.19 & UNS & 684.28 \\
or\_randxor\_k3\_n510\_m510 & UNS & 97.45 & UNS & 123.54 & UNS & 2.73 \\
pb\_300\_05\_lb\_17 & SAT & 54.99 & SAT & 174.99 & SAT & 23.86 \\
pb\_300\_09\_lb\_07 & SAT & 31.14 & SAT & 33.29 & SAT & 6.53 \\
pcmax\_scheduling\_m11\_1517\_6802\_UNSAT & UNS & 23.54 & UNS & 42.78 & UNS & 33.35 \\
pcmax\_scheduling\_m12\_8049\_55035\_SAT & SAT & 712.69 & SAT & 832.69 & TO & 3601.30 \\
pcmax\_scheduling\_m13\_1655\_9604\_UNSAT & UNS & 91.35 & UNS & 105.20 & UNS & 132.10 \\
pcmax\_scheduling\_m13\_2011\_12813\_UNSAT & UNS & 33.39 & UNS & 55.00 & UNS & 65.48 \\
pcmax\_scheduling\_m15\_2352\_13561\_SAT & TO & 3601.30 & TO & 3601.30 & SAT & 1230.79 \\
pcmax\_scheduling\_m19\_10199\_62102\_UNSAT & TO & 3601.31 & UNS & 2953.21 & UNS & 3079.06 \\
pcmax\_scheduling\_m19\_2974\_16501\_UNSAT & UNS & 87.05 & UNS & 99.64 & UNS & 25.23 \\
pcmax\_scheduling\_m24\_17855\_226744\_SAT & TO & 3601.30 & TO & 3601.30 & SAT & 2562.86 \\
pcmax\_scheduling\_m24\_24102\_255206\_SAT & TO & 3601.30 & TO & 3601.31 & TO & 3601.30 \\
pcmax\_scheduling\_m26\_6398\_62377\_UNSAT & UNS & 181.79 & UNS & 293.65 & UNS & 23.63 \\
pcmax\_scheduling\_m30\_14113\_167638\_UNSAT & TO & 3601.26 & TO & 3601.34 & UNS & 411.76 \\
pcmax\_scheduling\_m35\_32274\_371389\_SAT & TO & 3601.32 & TO & 3601.31 & SAT & 634.23 \\
pcmax\_scheduling\_m37\_28831\_324346\_SAT & TO & 3601.31 & TO & 3721.31 & TO & 3601.31 \\
pcmax\_scheduling\_m40\_26287\_324155\_SAT & SAT & 52.14 & SAT & 172.14 & SAT & 2159.83 \\
pcmax\_scheduling\_m43\_38782\_385402\_SAT & SAT & 188.99 & SAT & 255.94 & TO & 3601.30 \\
post\_cbmc\_aes\_ee\_r3\_noholes & TO & 3601.32 & TO & 3721.32 & UNS & 120.48 \\
preimage\_80r\_495m\_160h\_seed\_379 & SAT & 171.79 & SAT & 291.79 & SAT & 101.69 \\
Ptn\_7824\_b18 & SAT & 62.29 & SAT & 110.39 & SAT & 1.54 \\
qwh.50.1250.shuffled\_as.sat03\_1655 & SAT & 11.88 & SAT & 9.50 & SAT & 5.67 \\
qwh.60.1728.shuffled\_as.sat03\_1659 & SAT & 39.25 & SAT & 56.46 & SAT & 28.98 \\
rbsat\_v1150c84314gyes1 & TO & 3601.30 & TO & 3601.29 & TO & 3601.30 \\
rbsat\_v760c43649gyes3 & SAT & 44.27 & SAT & 72.33 & SAT & 29.56 \\
rbsat\_v760c43649gyes7 & SAT & 27.84 & SAT & 54.71 & SAT & 7.75 \\
rbsat\_v760c43649gyes9 & SAT & 48.64 & SAT & 78.39 & SAT & 3.33 \\
rbsat\_v945c61409gyes9\_sc2009 & SAT & 112.86 & SAT & 123.64 & SAT & 10.69 \\
REGRandom\_K3\_L3\_Seed25 & TO & 3601.66 & TO & 3601.35 & UNS & 49.93 \\
REGRandom\_K4\_L1\_Seed30 & TO & 3601.35 & TO & 3601.30 & UNS & 86.50 \\
REGRandom\_K4\_L2\_Seed35 & TO & 3601.31 & TO & 3601.34 & UNS & 945.89 \\
REGRandom\_K4\_L3\_Seed40 & TO & 3601.30 & TO & 3601.29 & UNS & 2006.16 \\
rook\_42\_0\_1 & TO & 3601.30 & TO & 3601.32 & UNS & 197.64 \\
rook\_56\_0\_0 & TO & 3601.31 & TO & 3601.31 & UNS & 574.96 \\
rook\_56\_1\_1 & TO & 3601.30 & TO & 3601.31 & UNS & 190.83 \\
rphp\_p8\_r160 & TO & 3601.32 & TO & 3721.32 & TO & 3601.35 \\
rphp\_p8\_r170 & TO & 3601.32 & TO & 3721.32 & TO & 3601.37 \\
Schur\_161\_5\_d38 & UNS & 257.29 & UNS & 305.97 & TO & 3601.39 \\
sgen1\_sat\_180\_100 & SAT & 50.34 & SAT & 43.63 & SAT & 4.47 \\
sgen1\_unsat\_121\_100 & TO & 3601.32 & TO & 3601.31 & TO & 3601.39 \\
SGI\_30\_60\_19\_60\_6\_dir.shuffled\_as.sat03\_112 & UNS & 469.65 & UNS & 441.57 & UNS & 643.66 \\
SGI\_30\_80\_26\_70\_4\_log.shuffled\_as.sat03\_208 & UNS & 879.47 & UNS & 642.14 & TO & 3601.39 \\
shuffling\_2\_s25242449\_of\_bench\_sat04\_727.53 & SAT & 266.86 & SAT & 386.86 & SAT & 2.64 \\
si2\_b03m\_m800\_03 & SAT & 34.49 & SAT & 154.49 & SAT & 3.53 \\
simon\_r16\_1 & TO & 3601.31 & SAT & 30.65 & SAT & 275.39 \\
simon\_r17\_0 & TO & 3601.32 & TO & 3601.31 & SAT & 407.54 \\
simon\_r18\_0 & TO & 3601.32 & SAT & 27.24 & SAT & 583.53 \\
simon\_r19\_1 & TO & 3601.32 & TO & 3601.31 & SAT & 469.95 \\
simon\_r20\_0 & SAT & 2445.14 & SAT & 2565.14 & SAT & 645.83 \\
simon\_r21\_0 & TO & 3601.31 & TO & 3601.30 & SAT & 670.39 \\
simon\_r22\_1 & TO & 3601.33 & SAT & 95.79 & SAT & 710.93 \\
simon\_r23\_1 & TO & 3601.31 & TO & 3601.33 & SAT & 604.03 \\
simon\_r24\_1 & TO & 3601.32 & TO & 3721.32 & SAT & 808.89 \\
simon\_r25\_0 & TO & 3601.35 & SAT & 11.96 & SAT & 816.93 \\
sokoban\_p16.sas.ex.15\_sc2016 & ERR & 84.75 & ERR & 85.29 & UNS & 253.43 \\
sokoban\_p20.sas.cr.25 & UNS & 1629.48 & UNS & 1663.74 & UNS & 392.03 \\
sokoban\_p20.sas.cr.33 & TO & 3601.32 & TO & 3601.31 & TO & 3601.44 \\
spg\_200\_316 & TO & 3601.31 & TO & 3601.31 & UNS & 114.94 \\
srhd\_sgi\_m37\_q446.25\_n35\_p30\_s33692332 & TO & 3601.32 & SAT & 45.78 & SAT & 735.19 \\
stable\_300\_0.1\_20\_98765432130020 & SAT & 9.97 & SAT & 26.58 & SAT & 2.59 \\
stb\_418\_125.apx\_1\_DC\_AD & UNS & 59.14 & UNS & 68.53 & UNS & 312.63 \\
stb\_418\_125.apx\_1\_DC\_ST & UNS & 24.15 & UNS & 33.94 & UNS & 132.58 \\
stb\_418\_125.apx\_2\_DC\_AD & UNS & 55.85 & UNS & 63.56 & UNS & 241.76 \\
stb\_495\_168.apx\_1\_DC\_AD & UNS & 21.24 & UNS & 43.44 & UNS & 53.86 \\
stb\_495\_168.apx\_2\_DC\_AD & UNS & 22.79 & UNS & 43.04 & UNS & 50.64 \\
stb\_531\_83.apx\_1\_DC\_ST & UNS & 37.70 & UNS & 43.77 & UNS & 77.28 \\
stb\_531\_83.apx\_2\_DC\_ST & UNS & 21.94 & UNS & 33.45 & UNS & 64.16 \\
stb\_588\_138.apx\_1\_DC\_AD & UNS & 39.04 & UNS & 50.24 & UNS & 164.09 \\
stb\_588\_138.apx\_1\_DC\_ST & UNS & 23.64 & UNS & 35.67 & UNS & 72.83 \\
StConn\_7\_128 & TO & 3601.30 & TO & 3601.32 & UNS & 566.59 \\
StConn\_8\_32 & TO & 3601.33 & TO & 3601.30 & UNS & 111.74 \\
sted5\_0x1e3\_20 & TO & 3601.33 & TO & 3601.31 & TO & 3601.36 \\
sted5\_0x24204\_50 & SAT & 495.20 & SAT & 615.20 & SAT & 10.43 \\
string\_compare\_safety\_cbmc\_unwinding\_900 & ERR & 260.54 & ERR & 257.30 & UNS & 347.93 \\
summle\_X11112\_steps6\_I1\_2\_2\_4\_4\_8\_25\_100 & SAT & 15.77 & SAT & 65.95 & SAT & 5.56 \\
summle\_X4044\_steps7\_I1\_2\_2\_4\_4\_8\_25\_100 & SAT & 16.17 & SAT & 78.94 & SAT & 4.03 \\
summle\_X4053\_steps8\_I1\_2\_2\_4\_4\_8\_25\_100 & SAT & 9.36 & SAT & 101.19 & SAT & 5.53 \\
T105.2.0 & TO & 3601.38 & TO & 3601.33 & UNS & 123.44 \\
test\_v7\_r17\_vr5\_c1\_s25451.smt2\_cvc4 & TO & 3601.37 & TO & 3601.30 & UNS & 2394.46 \\
Timetable\_C\_392\_E\_62\_Cl\_26\_S\_28 & SAT & 119.34 & SAT & 239.34 & SAT & 52.67 \\
tseitin\_d3\_n158 & TO & 3601.34 & TO & 3601.31 & UNS & 0.02 \\
tseitin\_d3\_n162 & TO & 3601.32 & TO & 3601.31 & UNS & 0.02 \\
tseitin\_d3\_n174 & TO & 3601.32 & TO & 3601.30 & UNS & 0.02 \\
tseitingrid6x200\_shuffled & TO & 3601.31 & TO & 3601.29 & UNS & 0.02 \\
tseitin\_grid\_n11\_m20 & TO & 3601.31 & TO & 3601.32 & TO & 3601.41 \\
two\_trees\_1023v & TO & 3601.33 & TO & 3601.32 & TO & 3601.40 \\
two\_trees\_511v & SAT & 706.94 & SAT & 726.05 & SAT & 989.49 \\
urq45 & UNS & 161.54 & UNS & 171.60 & UNS & 53.09 \\
urqh1c5x5.shuffled\_as.sat03\_1468.mis\_103 & TO & 3601.32 & TO & 3601.32 & TO & 3601.41 \\
VanDerWaerden\_2\_3\_14\_186 & UNS & 224.97 & UNS & 190.83 & UNS & 1483.58 \\
worker\_20\_40\_20\_0.95 & SAT & 0.91 & SAT & 1.04 & SAT & 0.04 \\
worker\_30\_60\_25\_0.9 & TO & 3601.31 & TO & 3601.31 & UNS & 0.04 \\
worker\_40\_80\_40\_0.9 & TO & 3601.32 & TO & 3601.30 & UNS & 0.08 \\
worker\_550\_550\_550\_0.3 & SAT & 271.24 & SAT & 272.14 & SAT & 4.98 \\
WS\_500\_16\_70\_10.apx\_1\_DC\_ST & UNS & 19.74 & UNS & 35.44 & UNS & 107.03 \\
WS\_500\_16\_70\_10.apx\_2\_DC\_AD & UNS & 50.39 & UNS & 59.80 & UNS & 118.05 \\
WS\_500\_16\_90\_70.apx\_2\_DC\_AD & UNS & 36.24 & UNS & 54.48 & UNS & 99.53 \\
x9\_08014.sat & UNS & 6.04 & UNS & 12.46 & UNS & 13.48 \\
x9\_08075.sat & UNS & 5.34 & UNS & 13.87 & UNS & 16.93 \\
x9\_09004.sat & UNS & 13.79 & UNS & 21.37 & UNS & 53.18 \\
x9\_09007.sat & UNS & 9.64 & UNS & 18.38 & UNS & 31.04 \\
x9\_09014.sat & UNS & 12.50 & UNS & 20.24 & UNS & 36.78 \\
x9\_09024.sat & UNS & 10.54 & UNS & 19.44 & UNS & 22.56 \\
x9\_09047.sat & UNS & 9.54 & UNS & 16.90 & UNS & 31.14 \\
x9\_09051.sat & UNS & 10.15 & UNS & 16.89 & UNS & 51.23 \\
x9\_09054.sat & SAT & 3.89 & SAT & 14.88 & SAT & 8.08 \\
x9\_09057.sat & UNS & 11.64 & UNS & 20.09 & UNS & 27.57 \\
x9\_09076.sat & UNS & 9.17 & UNS & 15.39 & UNS & 27.24 \\
x9\_09098.sat & UNS & 11.95 & UNS & 19.35 & UNS & 55.63 \\
x9\_10002.sat & UNS & 30.64 & UNS & 40.24 & UNS & 259.64 \\
x9\_10007.sat & UNS & 20.71 & UNS & 29.94 & UNS & 132.73 \\
x9\_10014.sat & SAT & 6.68 & SAT & 19.89 & SAT & 14.10 \\
x9\_10027.sat & SAT & 5.59 & SAT & 19.88 & SAT & 21.20 \\
x9\_10031.sat & UNS & 30.09 & UNS & 36.76 & UNS & 264.03 \\
x9\_10038.sat & SAT & 16.44 & SAT & 28.84 & SAT & 15.63 \\
x9\_10051.sat & UNS & 30.96 & UNS & 40.54 & UNS & 187.37 \\
x9\_10076.sat & UNS & 18.24 & UNS & 28.77 & UNS & 97.28 \\
x9\_10083.sat & UNS & 21.17 & UNS & 29.98 & UNS & 116.11 \\
x9\_10084.sat & UNS & 22.39 & UNS & 28.24 & UNS & 123.09 \\
x9\_10093.sat & UNS & 27.84 & UNS & 33.96 & UNS & 188.86 \\
x9\_10096.sat & UNS & 22.29 & UNS & 31.04 & UNS & 133.18 \\
x9\_10098.sat & SAT & 14.95 & SAT & 18.40 & SAT & 4.87 \\
x9\_11034.sat & SAT & 18.40 & SAT & 35.31 & SAT & 20.96 \\
x9\_11053.sat & SAT & 1.46 & SAT & 29.96 & SAT & 27.88 \\
x9\_11062.sat & SAT & 8.01 & SAT & 28.96 & SAT & 17.03 \\
x9\_11077.sat & SAT & 17.11 & SAT & 1.18 & SAT & 39.88 \\
x9\_11088.sat & SAT & 5.94 & SAT & 34.47 & SAT & 285.99 \\
x9\_11093.sat & SAT & 4.44 & SAT & 29.74 & SAT & 14.48 \\
x9\_11094.sat & SAT & 13.98 & SAT & 22.89 & SAT & 141.90 \\
x9\_12001.sat & SAT & 34.98 & SAT & 60.99 & SAT & 68.83 \\
x9\_12014.sat & SAT & 20.89 & SAT & 50.84 & SAT & 51.56 \\
x9\_12021.sat & SAT & 121.88 & SAT & 110.61 & SAT & 40.24 \\
x9\_12035.sat & SAT & 36.96 & SAT & 51.19 & SAT & 115.46 \\
x9\_12063.sat & SAT & 39.28 & SAT & 62.66 & SAT & 96.99 \\
x9\_12087.sat & SAT & 90.64 & SAT & 100.94 & SAT & 40.37 \\
x9\_12092.sat & SAT & 36.94 & SAT & 61.44 & SAT & 61.23 \\
x9\_12098.sat & SAT & 111.59 & SAT & 106.99 & SAT & 31.30 \\
\bottomrule
\end{xltabular}
\end{center}

